Structured Light with Redundancy Codes

Structured light (SL) systems acquire high-fidelity 3D geometry with active illumination projection. Conventional systems exhibit challenges when working in environments with strong ambient illumination, global illumination and cross-device interference. This paper proposes a general-purposed technique to improve the robustness of SL by projecting redundant optical signals in addition to the native SL patterns. In this way, projected signals become more distinguishable from errors. Thus the geometry information can be more easily recovered using simple signal processing and the ``coding gain" in performance is obtained. We propose three applications using our redundancy codes: (1) Self error-correction for SL imaging under strong ambient light, (2) Error detection for adaptive reconstruction under global illumination, and (3) Interference filtering with device-specific projection sequence encoding, especially for event camera-based SL and light curtain devices. We systematically analyze the design rules and signal processing algorithms in these applications. Corresponding hardware prototypes are built for evaluations on real-world complex scenes. Experimental results on the synthetic and real data demonstrate the significant performance improvements in SL systems with our redundancy codes.

==> intro_bk.tex <==
% Jian's version, don't delete
\IEEEPARstart{S}{tructured} light (SL) is a kind of widely used active 3D imaging method that requires a projector to project designed patterns and a camera to capture images in which the warped patterns over the target to recover the 3D information of the scanned objects~\cite{boyer1987color,geng2011structured,gupta2011structured,gupta2013structured,zhan2017high,liu2017high,jiang2018three}. 
%,morano1998structured,zhang2006novel,chen2008vision,salvi2010state,feng2019fringe,saragadam2019micro,zhang2008three,
Commercial SL imaging technologies are further subdivided into two series，single pattern methods and multiple pattern approaches，based on the number of projected patterns. 
Single pattern methods continuously project a static pattern to encode the scenarios, which is especially suitable for real-time scanning of dynamic objects, such as the technologies adopted in Microsoft Kinect V1 and Intel RealSense~\cite{boyer1987color,freedman2012depth,khoshelham2011accuracy,khoshelham2012accuracy,zhang2012review,sarbolandi2015kinect}. 
%,vuylsteke1990range,je2004high,geng2011structured,geng1996rainbow,
Multiple pattern approaches require a light emitting device to project a number of patterns so that each projector pixel is encoded along the time axis~\cite{posdamer1982surface,geng2011structured,jiang2018three,liu2010dual,saragadam2019micro}. One of mainstream case in the multiple pattern field is binary or gray coding approach where each pixel is labelled by an 10 bit unique address~\cite{sansoni1999three,zhang20123,zheng2017phase,wu2019high,wu2019highcyclic,wang2020dynamic}, depending on projector resolution, for each pixel of the projector. After one-to-one correspondence between the projector plane and camera image is established, the depth of an object surface point can be estimated by the triangulation principle. 

In multiple patterns SL, the column/row coordinates of each pixel are encoded through modulation~\cite{srinivasan1984automated,huang2006fast,Garcia2012Consistent,An2016Pixel} 
%liu2010dual,geng2011structured,chen2008modulated,wang2011period,zhang2006high,
and the theoretically accuracy of these scanners can almost reach tens of microns in ideal scan environment. However, as an active imaging technique, SL suffers from various challenges in real scan scenarios, such as ambient light, global illumination, and interference.
Strong ambient light severely decrease the Signal Noise Ratio (SNR), leading to significant performance degradation of SL 3D imaging, especially in outdoor daylight scenarios ~\cite{gupta2013structured} or high speed scanning cases with limited exposure time period. 
Global illumination, including inter-reflections, diffusion and sub-surface scattering, providing indirect illumination to the current observation, seriously affect the intensity of the ROI, introducing reconstruction errors~\cite{gupta2011structured,gupta2015phasor,gupta2012micro}. 
Interference between multiple structured light sensors ~\cite{maimone2012reducing} or within a single structured light setup cause redirection of projected light to form multiple paths from projector to camera besides the direct light path of projector to target to camera. Bimodal multi-path interference is an especially vital and unavoidable phenomenon exsiting in any scanning based 3D imaging modalities, where a target surface includes a step edge, resulting in pixels of the camera collecting light from a foreground and background surface~\cite{zhang2019causes}.


%but as an active imaging technique, SL is susceptible to errors under ambient illumination and distortions caused by the redirection of the projected light to form multiple paths from projector to camera besides the direct path of projector to target to camera~\cite{wang2012robust,nayar2006fast,gupta2015phasor,o2014temporal,gupta2012micro,SongA}. It is a common problem and one of great interest to researchers because of the potentially catastrophic effects on scans. The same problem can be found in a range of 3D imaging modalities, such as time-of-flight (ToF) where light will reflect off specular surfaces onto neighboring surface points before reflecting back to the camera.


In this paper, we propose to use redundancy to solve these problems. It can… if the frame rate of the system allows. Three kinds of codes are applied and in-depth analysis is provided.

Moreover, these methods can be extended to direct ToF directly, since TOF is also susceptible to errors under ambient illumination, global illumination and multi-path interference.


We summarize our contributions in the following. 
(1) We adapt these channel encoding/decoding ideas from the communication community to an SL system by its uniqueness (noise resources, the difference of performance under photon noise and camera's readout noise, limited search space enabling soft decoding, how to arrange codes in the projector's pattern, which N-ary codes to use, adaptive SL uses which code, source encoding)
(2) We propose three kinds of encoding.
(3) We use simulations and real-world devices to validate them.

\textbf{Limitations}. Needs higher frame rate (we provide choices of difference encoding for different frame rate systems). Limited to static objects.  

% end of Jian's version
